Distributing Quantum Circuits Using Teleportations

Scalability is currently one of the most sought-after objectives in the field of quantum computing. Distributing a quantum circuit across a quantum network is one way to facilitate large computations using current quantum computers. In this paper, we consider the problem of distributing a quantum circuit across a network of heterogeneous quantum computers, while minimizing the number of teleportations (the communication cost) needed to implement gates spanning multiple computers. We design two algorithms for this problem. The first, called Local- Best, initially distributes the qubits across the network, then tries to teleport qubits only when necessary, with teleportations being influenced by gates in the near future. The second, called Zero- Stitching, divides the given circuit into sub-circuits such that each sub-circuit can be executed using zero teleportations and the teleportation cost incurred at the borders of the sub-circuits is minimal. We evaluate our algorithms over a wide range of randomly-generated circuits as well as known benchmarks, and compare their performance to prior work. We observe that our techniques outperform the prior approach by a significant margin (up to 50%).

==> Hardness.tex <==
\section{NP-Hardness Proof}

\begin{itemize}
    \item Reduction from graph minimum bisection problem. 
\end{itemize}
